Blinded by Generated Contexts: How Language Models Merge Generated and Retrieved Contexts When Knowledge Conflicts?

While auxiliary information has become a key to enhancing Large Language Models (LLMs), relatively little is known about how LLMs merge these contexts, specifically contexts generated by LLMs and those retrieved from external sources. To investigate this, we formulate a systematic framework to identify whether LLMs' responses are attributed to either generated or retrieved contexts. To easily trace the origin of the response, we construct datasets with conflicting contexts, i.e., each question is paired with both generated and retrieved contexts, yet only one of them contains the correct answer. Our experiments reveal a significant bias in several LLMs (GPT-4/3.5 and Llama2) to favor generated contexts, even when they provide incorrect information. We further identify two key factors contributing to this bias: i) contexts generated by LLMs typically show greater similarity to the questions, increasing their likelihood of being selected; ii) the segmentation process used in retrieved contexts disrupts their completeness, thereby hindering their full utilization in LLMs. Our analysis enhances the understanding of how LLMs merge diverse contexts, offers valuable insights for advancing current LLM augmentation methods, and highlights the risk of generated misinformation for retrieval-augmented LLMs.

==> Experiment_Setup_old.tex <==
\section{Experiment Settings} \label{Experimental Setup}


To investigate how LLMs merge generated and retrieved contexts, we conduct experiments on the open-domain question answering task, which is a representative knowledge-intensive task.
We construct (question, a generated context, a retrieved context) triples where only one of the contexts contains the correct answer.
LLMs are required to answer the question based on concatenated generated and retrieved contexts, and then we evaluate which context LLMs rely on.
Figure \ref{fig_dataset_construction} illustrates the comprehensive framework for constructing context-conflicting datasets and evaluating context preference.


\textbf{Models.} We analyze several state-of-the-art LLMs. 
The GPT series, including GPT 4 (\textit{gpt-4-0613}) and GPT-3.5 (\textit{gpt-3.5-turbo-0613}), was accessed via the OpenAI API.
Additionally, we evaluate open-source models such as Llama2-7b (\textit{Llama-2-7b-chat}) and Llama2-13b (\textit{Llama-2-13b-chat}) \citep{touvron2023llama}.


\subsection{Datasets} \label{subsets}

\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{0.6\textwidth}
        \includegraphics[width=1\linewidth]{diagram/dataset.pdf}
        \subcaption{Process of constructing context-conflicting subsets}
        \label{fig_dataset_construction_a}
    \end{minipage} \hspace{10mm}
    \begin{minipage}[t]{0.28\textwidth}
        \includegraphics[width=1\linewidth]{diagram/evaluation.pdf}
        \subcaption{Evaluation of context preference}
        \label{fig_dataset_construction_b}
    \end{minipage}
    \caption{The framework of constructing context-conflicting subsets (\ref{fig_dataset_construction_a}) and evaluating context preference (\ref{fig_dataset_construction_b}).}
    \label{fig_dataset_construction}
\end{figure*}

Our experiments are conducted on two widely utilized open-domain question-answering benchmarks: NaturalQuestions (NQ) \citep{kwiatkowski2019natural} and TriviaQA (TQA) \citep{joshi2017triviaqa}, which contain questions and corresponding golden answers.
We construct context-conflicting subsets using the following criteria: 
(1) Each question corresponds to a generated context and a retrieved context;
(2) Only one of these contexts provides the correct answer, while the other provides an incorrect answer.
The detailed steps are as follows:

\textbf{Step1. Prepare retrieved and  generated contexts.} 
As depicted in Figure \ref{fig_dataset_construction_a} step 1, a retrieved context and a generated context are prepared for each question.
We incorporate just a single instance for every source of context in order to streamline the scenario and facilitate the construction of conflicts.

We employ Contriever \citep{izacard2021unsupervised} as the retriever.
It is an effective off-the-shelf retrieval model that is widely used in various retrieval-augmented methods \citep{shi2023replug, liu2023lost,ram2023context}.
The top-1 document retrieved by Contriever from Wikipedia is considered as the retrieved context.

Following GenRead \citep{yu2022genread}, we instruct the generator to produce a context based on the given question with a prompt like \textit{``Generate a background context from Wikipedia to answer the given question.\{\#question\}''}.
However, we note that the generated context tends to be significantly longer than the retrieved context which consists of a title and a 100-word text. 
The disparity in length between the two contexts could potentially influence the context preference.
To ensure a fair comparison, we incorporate \textit{``Keep the length of the document around n words''} in the prompt to regulate the length of the generated context.
Since current LLMs struggle to precisely control the length of the output, we generate multiple contexts with different values of $n$ and select the context that is closest in length to the retrieved context.

As shown in Table \ref{table_length}, the final generated context exhibits a comparable length to the retrieved context, with the average difference in length being less than 3\%.
The detailed length distribution is provided in Appendix \ref{appendix_length_distribution}.
Table \ref{table_length} also illustrates the recall of contexts, which is the ratio of the context containing the golden answer strings.
The generated contexts demonstrate a higher recall rate than retrieved contexts, with the exception of Llama2-7b. 
This suggests that LLMs are effective as knowledge generators, aligning with previous works \citep{yu2022genread,chen2023beyond}.

\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{Context} & \multicolumn{2}{c}{NQ} & \multicolumn{2}{c}{TQA} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & Length & Recall & length & Recall \\
    \midrule
    Retrieved & 107.3 & 0.403 & 106.3 & 0.528 \\
    \midrule
    GPT 4 & 108.0 & 0.659 & 107.2 & 0.828 \\
    GPT 3.5 & 106.0 & 0.568 & 104.9 & 0.779 \\
    Llama2-13b & 110.1 & 0.441 & 105.5 & 0.657 \\
    Llama2-7b & 104.0 & 0.389  & 102.6 & 0.606 \\
    \bottomrule
\end{tabular}
    \end{adjustbox}
    \caption{Average lengths and recall of the generated and retrieved contexts. Length is measured in the number of words after punctuation removal. Recall is the ratio of the context containing the golden answer strings.}
    \label{table_length}
\end{table}


\textbf{Step2. Produce candidate answer for each context.} 
\textcolor{black}{
To extract context-conflicting subsets, it is necessary to first ascertain the candidate answers provided in each context, as shown at step 2 in Figure \ref{fig_dataset_construction_a}.
We employ the reader to answer the question solely based on the generated context, yielding candidate answer referred to as Gen-Ans. 
Similarly, by answering question solely based on the retrieved context, we obtain Ret-Ans.
}
Following \citet{yu2022genread}, the reader use the prompt \textit{``Refer to the context below and answer the following question with just one entity. context: \{\#contexts\} Question: \{\#question\} The answer is''}.

Readers may sometimes abstain from providing an answer, issuing responses like ``unknown'' when they cannot get relevant information from the provided contexts. 
We exclude examples where either Gen-Ans or Ret-Ans is an abstention, as no conflict arises in such cases.

A potential concern may be whether the candidate answer truly originates from the input context rather than LLMs' parameter knowledge. 
Recent studies \citep{chen2022rich,xie2023knowledgeconflicts} have found that when given a context, LLMs highly receptive to the input context rather than resorting to parameter knowledge. 
\textcolor{black}{To further ensure that the candidate answer comes from the corresponding context, we retain only those instances where the context explicitly contains the candidate answer string.}



\textbf{Step3. Extract context-conflicting subsets.} 
Step 3 in Figure \ref{fig_dataset_construction_b} illustrates how we extract context-conflicting subsets based on the candidate answers.
Firstly, we use Exact Match (EM) \citep{yu2022genread} score to evaluate whether the candidate answers are correct.
Concretely, an answer is considered correct if and only if its normalized form has a match in the golden answer list provided in the dataset.
Subsequently, context-conflicting subsets are extracted based on the correctness of these candidate answers.
For instance, in the NQ dataset, the group of examples where all Gen-Ans are correct, and all Ret-Ans are incorrect, make up NQ-AIG (AIG stands for \textbf{A}nswer \textbf{I}n \textbf{G}enerated context). Conversely, the group of cases where all Gen-Ans are incorrect and all Ret-Ans are correct, make up NQ-AIR (AIR stands for \textbf{A}nswer \textbf{I}n \textbf{R}etrieved context).

\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lrrrr}
        \toprule
    	\multirowcell{2.5}{Backbone\\ LLM} & \multicolumn{2}{c}{NQ (3610)} & \multicolumn{2}{c}{TQA (11313)} \\
        \cmidrule(lr){2-3}  \cmidrule(lr){4-5}
        & NQ-AIG & NQ-AIR & TQA-AIG & TQA-AIR \\
    	\midrule
        GPT 4  & 331 & 238  & 946 & 358 \\
        GPT 3.5  & 379 & 279  & 1357 & 567 \\
        Llama2-13b  & 439 & 419  & 1648 & 1201 \\
        Llama2-7b & 432 & 406 & 1737 & 1488 \\
        \midrule
        Avg. Proportion  & 10.9\% & 9.3\%  & 12.6\% & 8.0\% \\
    	\bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The data quantities of the constructed subsets for different LLMs. NQ and TQA refer to the original complete test sets. The proportion of the subset to the corresponding complete dataset is shown in the last row. Detailed analysis is shown in section \ref{subsets}}
    \label{Statistics}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{../paper/new_pic/prompt_similar_length_4/main_preference_wo_others.pdf}
    \caption{Answer ratio of LLMs when we provide both the self-generated and retrieved context. Gen-Ans and Ret-Ans refer to the candidate answers supported by the generated context and retrieved context, respectively. In the NQ-AIR and TQA-AIR datasets, Gen-Ans is incorrect, whereas Ret-Ans is correct. Conversely, in the NQ-AIG and TQA-AIG datasets, Gen-Ans is correct, and Ret-Ans is incorrect, as explained in section \ref{subsets}.}
    \label{preference}
\end{figure*}


\begin{table*}[t]
    \centering
    \begin{adjustbox}{max width=\textwidth} %
    \begin{tabular}{llrrrrrr}
        \toprule
        Backbone LLMs & Context & NQ & NQ-AIG & NQ-AIR & TQA & TQA-AIG & TQA-AIR \\

        \midrule
        \multirow{3}{*}{GPT 4} & Generated-only & 39.14 & 100.0 & 0.0 & 70.93 & 100.0 & 0.0 \\
         & Retrieved-only & 28.81 & 0.0 & 100.0  & 54.09 & 0.0 & 100.0	 \\
         & Generated + Retrieved & \textbf{39.81} & 91.54 & 14.29  & \textbf{71.08} & 94.08 & 18.44 \\

        \midrule
        \multirow{3}{*}{GPT 3.5} & Generated-only & 32.27 & 100.0 & 0.0   & \textbf{64.34} & 100.0 & 0.0	 \\
         & Retrieved-only & 25.46 & 0.0 & 100.0  & 52.94 & 0.0 & 100.0 \\
         & Generated + Retrieved & \textbf{32.66} & 94.46 & 13.26  & 64.30 & 93.96 & 19.58 \\
        
        \midrule
        \multirow{3}{*}{Llama2-13b} & Generated-only & 26.15 & 100.0 & 0.0 & 56.12 & 100.0 & 0.0 \\
         & Retrieved-only & 25.60 & 0.0 & 100.0  & 52.20 & 0.0 & 100.0 \\
         & Generated + Retrieved & \textbf{27.76} & 89.52 & 17.66 & \textbf{57.45} & 91.81 & 20.23 \\

        \midrule
        \multirow{3}{*}{Llama2-7b} & Generated-only & \textbf{23.10} & 100.0 & 0.0  & \textbf{48.19} & 100.0 & 0.0 \\
         & Retrieved-only & 22.41 & 0.0 & 100.0 & 46.03 & 0.0 & 100.0 \\
         & Generated + Retrieved & 22.47 & 67.13 & 23.40  & 46.95 & 80.08 & 21.64 \\

        \bottomrule
        
    \end{tabular}
    \end{adjustbox}

    \caption{The EM score with different sources of context. A detailed introduction of the subsets in \ref{subsets}. In this setup, both the generator and the reader are the backbone LLM. The values 0 and 100 in the table are attributed to the definition of the AIG and AIR subsets, as explained in Section \ref{subsets}. }
    \label{correct_ratio}
\end{table*}

\subsection{Statistics of Datasets}

As a result, for every LLM (work as both reader and generator here), we constructed four context-conflicting subsets NQ-AIG, NQ-AIR, TQA-AIG, and TQA-AIR.
The statistics of each subset are detailed in Table \ref{Statistics}, which reveals that the AIG and AIR conflicting subsets account for a noticeable proportion in the complete test sets. 
This observation indicates that a considerable number of questions have only one context type that contains the correct answer, highlighting the importance of examining LLM behavior in the presence of contextual conflicts.
Additionally, GPT 4 has fewer context-conflicting instances than other LLMs, as shown in Table \ref{Statistics}.
This is because it has higher proportion of instances where it correctly answers using either only retrieved context or only generated context.










\subsection{Evaluation} \label{evaluation}
We assess the context preference through a question-answering task, where the reader is required to answer questions based on both generated and retrieved contexts on the proposed context-conflicting subsets, as shown in Figure \ref{fig_dataset_construction_b}.
We employed a randomized input sequence for contexts to mitigate the impact of order \citep{xie2023knowledgeconflicts,liu2023lost,lu2021fantastically}.
Appendix \ref{section_order} shows the results with other orders and demonstrates similar conclusion.

To reveal which context LLMs actually rely on, We compute the proportion of answers that exactly match candidate answers supported by different contexts seperately.
It is also possible that the predicted answer does not exactly match either Gen-Ans or Ret-Ans, due to the limitations of exactly matching.
We consider such answers as ``Others'' which occur with a relatively low probability and do not affect the conclusions regarding context preference, as shown in Section \ref{Results and Discussing}.
Additionally, to eliminate the numerical impact of the  ``Others'', we introduce the generation ratio:
$$\text{Generation Ratio} = \frac{f_\text{Gen-Ans} - f_\text{Ret-Ans}}{f_\text{Gen-Ans}+f_\text{Ret-Ans}}$$
where $f_\text{Gen-Ans}$ is the frequency of choosing Gen-Ans and $f_\text{Gen-Ans}$ is the frequency of choosing Ret-Ans.
The denominator serves to normalize the generation ratio to the range of [-1,1].
A positive generation ratio denotes a preference for generated context and the absolute value represents the magnitude of the preference.




        
     
     

\begin{figure}[t]
        \centering
        \begin{minipage}[t]{0.5\textwidth}
            \includegraphics[width=1\linewidth]{../paper/new_pic/prompt_similar_length_4/new_generation_heatmap_nq_air.pdf}
            \label{fig_heatmap_air}
        \end{minipage}
    \caption{The generation ratio (\%) with different (Reader, Generator) pairs on NQ-AIR.}
    \label{preference_reader_generator}
\end{figure}









==> case.tex <==

\begin{figure}[t]
    \begin{mdframed}[
        backgroundcolor=gray!10,    %
        roundcorner=10pt,           %
        frametitlebackgroundcolor=gray!20,  %
        frametitlerule=true,        %
        frametitlealignment=\center, %
        innertopmargin=10pt,        %
        innerbottommargin=10pt,     %
        innerleftmargin=10pt,       %
        innerrightmargin=10pt,      %
        splitbottomskip=10pt        %
    ]
    
    question: what is bermuda competing in the winter olympics?
    
    \end{mdframed}
    
    \begin{mdframed}[
        backgroundcolor=gray!10,    %
        roundcorner=10pt,           %
        frametitlerule=true,        %
        innertopmargin=10pt,        %
        innerbottommargin=10pt,     %
        innerleftmargin=10pt,       %
        innerrightmargin=10pt       %
    ]
    
    Generated Document: Due to the lack of winter sports infrastructure in Bermuda, athletes representing the country in \textcolor{orange}{skeleton} typically train and compete abroad.
    
    Retrieved Document: Bermuda was represented by one athlete, \textcolor{purple}{cross-country skier} Tucker Murphy, who finished his only event in 104th place.
    
    answer: \textcolor{orange}{skeleton}
    \end{mdframed}

    \caption{The case of knowledge conflicting}
    \label{case}
\end{figure}




==> color.tex <==
\definecolor{bg_gray}{RGB}{247, 247, 247}

\definecolor{tea_green}{RGB}{214, 234, 193}
\definecolor{hint_green}{RGB}{226,246,209}
\definecolor{Madang}{RGB}{190,235,159}
\definecolor{yellow_green}{RGB}{198,222,119}
\definecolor{link_water}{RGB}{221, 232, 250}
\definecolor{celestial_blue}{RGB}{52, 152, 219}
\definecolor{shakespeare}{RGB}{85, 154, 193}
\definecolor{buttermilk}{RGB}{255,242,174}
\definecolor{chardonnay}{RGB}{250,196,114}
\definecolor{rajah}{RGB}{253,180,98}
\definecolor{fog}{RGB}{213, 193, 234}
\definecolor{melon}{RGB}{254,191,181}
\definecolor{sundown}{RGB}{249, 180, 181}
\definecolor{mona_lisa}{RGB}{246,152,134}
\definecolor{salmon}{RGB}{242,131,107}


\definecolor{saltpan}{RGB}{238, 243, 232}
\definecolor{aqua_spring}{RGB}{232, 243, 232}
\definecolor{tea_green}{RGB}{214, 234, 193}
\definecolor{Madang}{RGB}{190,235,159}
\definecolor{fringy_flower}{RGB}{194, 234, 193}
\definecolor{aero_blue}{RGB}{193, 234, 213}
\definecolor{pixie_green}{RGB}{183,214,170}
\definecolor{french_pass}{RGB}{195,232,246}
\definecolor{ice_cold}{RGB}{169,232,220}
\definecolor{pale_turquoise}{RGB}{172,240,242}
\definecolor{cruise}{RGB}{179,226,205}
\definecolor{sail}{RGB}{163,205,235}
\definecolor{spindle}{RGB}{179,205,227}
\definecolor{link_water}{RGB}{221, 232, 250}
\definecolor{periwinkle}{RGB}{203,213,232}
\definecolor{zanah}{RGB}{220, 233, 213}
\definecolor{frostee}{RGB}{217, 231, 214}
\definecolor{opal}{RGB}{199, 221, 211}
\definecolor{jet_stream}{RGB}{188, 214, 210}
\definecolor{skeptic}{RGB}{153, 187, 167}
\definecolor{hint_green}{RGB}{226,246,209}
\definecolor{snow_flurry}{RGB}{230,245,201}
\definecolor{surf_crest}{RGB}{205,230,208}
\definecolor{yellow_green}{RGB}{198,222,119}
\definecolor{cream}{RGB}{255,255,204}
\definecolor{pale_prim}{RGB}{255,255,179}
\definecolor{spring_sun}{RGB}{242,243,195}
\definecolor{portafino}{RGB}{245,237,160}
\definecolor{cream_brulee}{RGB}{255, 229, 151}
\definecolor{dairy_cream}{RGB}{254,226,189}
\definecolor{champagne}{RGB}{254,217,166}
\definecolor{chardonnay}{RGB}{250,196,114}
\definecolor{manhattan}{RGB}{226,180,125}
\definecolor{rajah}{RGB}{253,180,98}
\definecolor{early_dawn}{RGB}{252,243,218}
\definecolor{egg_shell}{RGB}{238, 234, 215}
\definecolor{selago}{RGB}{243, 232, 243}
\definecolor{quartz}{RGB}{219,223,238}
\definecolor{languid_lavender}{RGB}{222,203,228}
\definecolor{watusi}{RGB}{254,221,207}
\definecolor{coral_andy}{RGB}{243,204,205}
\definecolor{cosmos}{RGB}{248,209,210}
\definecolor{melon}{RGB}{254,191,181}
\definecolor{azalea}{RGB}{234, 193, 194}
\definecolor{beauty_bush}{RGB}{235, 185, 179}
\definecolor{sundown}{RGB}{249, 180, 181}
\definecolor{mona_lisa}{RGB}{246,152,134}
\definecolor{salmon}{RGB}{242,131,107}


\definecolor{summer_sky}{RGB}{58, 151, 233}
\definecolor{chateau_green}{RGB}{72, 179, 96}
\definecolor{matisse}{RGB}{25, 104, 167}
\definecolor{allports}{RGB}{31, 106, 125}
\definecolor{sun_shade}{RGB}{255, 144, 68}
\definecolor{flamingo}{RGB}{237, 88, 85}
\definecolor{studio}{RGB}{128, 91, 160}



\definecolor{maya_blue}{RGB}{102, 204, 255}
\definecolor{feijoa}{RGB}{178,223,138}
\definecolor{sushi}{RGB}{117, 168, 47}
\definecolor{norway}{RGB}{158, 194, 132}
\definecolor{japanese_laurel}{RGB}{53, 116, 40}
\definecolor{see_green}{RGB}{161,228,195}
\definecolor{monte_carlo}{RGB}{135,204,194}
\definecolor{granny_smith_apple}{RGB}{150,214,150}
\definecolor{moss_green}{RGB}{170,216,176}
\definecolor{chateau_green}{RGB}{72, 179, 96}
\definecolor{opal}{RGB}{164,207,190}
\definecolor{acapulco}{RGB}{117, 170, 148}
\definecolor{viridian}{RGB}{55, 137, 122}
\definecolor{amazon}{RGB}{56, 123, 84}
\definecolor{asparagus}{RGB}{123, 160, 91}
\definecolor{fruit_salad}{RGB}{91, 160, 94}
\definecolor{puerto_rico}{RGB}{72, 179, 150}
\definecolor{mountain_meadow}{RGB}{0, 163, 136}
\definecolor{matisse}{RGB}{25, 104, 167}
\definecolor{allports}{RGB}{31, 106, 125}
\definecolor{astral}{RGB}{55, 111, 137}
\definecolor{spring_leaves}{RGB}{46, 83, 117}
\definecolor{biscay}{RGB}{44, 62, 80}
\definecolor{midnight}{RGB}{0, 29, 50}
\definecolor{amethyst}{RGB}{153, 102, 204}
\definecolor{studio}{RGB}{128, 91, 160}
\definecolor{tapestry}{RGB}{194, 109, 132}
\definecolor{atomic_tangerine}{RGB}{255, 153, 102}
\definecolor{amber}{RGB}{255, 191, 0}
\definecolor{casablanca}{RGB}{244, 178, 84}
\definecolor{california}{RGB}{233, 140, 58}
\definecolor{tomato}{RGB}{255, 97, 56} 
\definecolor{alizarin}{RGB}{233, 58, 64}



\definecolor{linen}{RGB}{251, 239, 227}
\definecolor{double_pearl_lusta}{RGB}{253, 242, 208}
\definecolor{oasis}{RGB}{253, 242, 208}
\definecolor{milan}{RGB}{255, 254, 169}
\definecolor{texas}{RGB}{245, 232, 123}
\definecolor{maize}{RGB}{249, 212, 156}

\definecolor{turmeric}{RGB}{211, 178, 76}
\definecolor{saffron}{RGB}{249,193,62}
\definecolor{my_sin}{RGB}{255, 176, 59}
\definecolor{tree_poppy}{RGB}{246, 154, 27}
\definecolor{jaffa}{RGB}{240, 131, 58}
\definecolor{crusta}{RGB}{254, 127, 44}
\definecolor{tahiti_gold}{RGB}{223, 102, 36}
\definecolor{outrageous_orange}{RGB}{255, 100, 45}
\definecolor{safety_orange}{RGB}{254, 106, 0}


\definecolor{azalea}{RGB}{251, 196, 196}
\definecolor{oyster_pink}{RGB}{238,206,205} 
\definecolor{coral_candy}{RGB}{242,208,205} 
\definecolor{baby_pink}{RGB}{246, 194, 192}
\definecolor{petite_orchid}{RGB}{223, 157, 155}
\definecolor{apricot}{RGB}{241,140,122}
\definecolor{NY_pink}{RGB}{228,136,113}
\definecolor{carmine_pink}{RGB}{231, 76, 60}
\definecolor{deep_carmine_pink}{RGB}{236, 50, 67}

\definecolor{wewak}{RGB}{244, 143, 150}
\definecolor{light_coral}{RGB}{244, 127, 123}
\definecolor{bittersweet}{RGB}{255,111,105}
\definecolor{carnation}{RGB}{245, 80, 86}
\definecolor{flamingo}{RGB}{237, 88, 85}
\definecolor{sunset_orange}{RGB}{242,89,75}
\definecolor{ku_crimson}{RGB}{243, 0, 25}
\definecolor{amaranth}{RGB}{234,46,73}
\definecolor{valencia}{RGB}{214, 87, 70}
\definecolor{chilean_fire}{RGB}{215, 87, 44}
\definecolor{mexican_red}{RGB}{170, 41, 37}



\definecolor{napa}{RGB}{163, 154, 137}

\definecolor{athens_gray}{RGB}{236, 240, 241}
\definecolor{gallery}{RGB}{240,240,240}
\definecolor{mercury}{RGB}{230,230,230}
\definecolor{platinum}{RGB}{228,228,228}
\definecolor{silver}{RGB}{191,191,191}
\definecolor{aluminum}{RGB}{153,153,153}
\definecolor{ship_gray}{RGB}{77,77,77}
\definecolor{tuatara}{RGB}{67, 67, 67}

\definecolor{malibu}{RGB}{110, 180, 240}
\definecolor{celestial_blue}{RGB}{52, 152, 219}
\definecolor{curious_blue}{RGB}{41, 128, 185}
\definecolor{french_blue}{RGB}{0, 112, 182}
\definecolor{matisse}{RGB}{25, 104, 167}
\definecolor{shakespeare}{RGB}{85, 154, 193}
\definecolor{seagull}{RGB}{128,177,211}
\definecolor{jelly_bean}{RGB}{45, 126, 150}
\definecolor{venice_blue}{RGB}{87, 135, 105}
\definecolor{boston_blue}{RGB}{68, 147, 161}

\definecolor{turquoise}{RGB}{41,217,194}
\definecolor{java}{RGB}{2,190,196}
\definecolor{riptide}{RGB}{141,211,199}
\definecolor{mountain_meadow}{RGB}{0, 163, 136}
\definecolor{free_speech_aquamarine}{RGB}{0, 156, 114}

\definecolor{cosmic_latte}{RGB}{222, 247, 229}
\definecolor{chinook}{RGB}{163, 232, 178}
\definecolor{padua}{RGB}{121, 189, 143}
\definecolor{ocean_green}{RGB}{79, 176, 112}
\definecolor{pastel_green}{RGB}{107, 227, 135}
\definecolor{chateau_green}{RGB}{69, 191, 85}
\definecolor{RoyalBlue}{RGB}{69, 191, 85}
\definecolor{pigment_green}{RGB}{0, 175, 79}
\definecolor{fern}{RGB}{101,197,117}
\definecolor{killarney}{RGB}{56, 113, 66}


==> def.tex <==
\DeclareMathOperator{\similarity}{sim}
\DeclareMathOperator{\reader}{reader}
\DeclareMathOperator{\generator}{generator}

